The case for an EIC Theory Alliance: Theoretical Challenges of the EIC

We outline the physics opportunities provided by the Electron Ion Collider (EIC). These include the study of the parton structure of the nucleon and nuclei, the onset of gluon saturation, the production of jets and heavy flavor, hadron spectroscopy and tests of fundamental symmetries. We review the present status and future challenges in EIC theory that have to be addressed in order to realize this ambitious and impactful physics program, including how to engage a diverse and inclusive workforce. In order to address these many-fold challenges, we propose a coordinated effort involving theory groups with differing expertise is needed. We discuss the scientific goals and scope of such an EIC Theory Alliance.

==> sat.tex <==


With its access to high energies, electron and light ion polarization, a wide range of nuclear species, and unprecedented DIS luminosities \cite{Accardi:2012qut,AbdulKhalek:2021gbh}, the EIC has the potential to reveal and establish the properties of gluon saturation, including its effects on proton spin and the physics of strong QCD color fields with unprecedented precision. Indeed, this discovery and characterization was deemed to be a principal objective of EIC science in the National Academy of Sciences report \cite{NAP25171}. 

At short distances, the proton can be viewed as a collection of weakly interacting quarks and gluons, commonly referred to as partons, each carrying a fraction $x$ of the proton momentum. The parton picture is expected to break down, however, when the resolution of the probe is on the order the proton size and confinement forces are at play. On the other hand, at sufficiently small $x$, the proton wave function is characterized by a rapid rise of the number of ``wee'' gluons up to a point where many-body recombination and screening effects become important, leading to  saturation of the gluon distribution. This novel many-body regime of QCD, characterized by strong non-linear gauge fields, can be explored in the framework of the Color Glass Condensate effective field theory (CGC)~\cite{Gelis:2010nm}. Such effects are strongly enhanced in nuclei, as reflected in the $Q_S^2\propto A^{1/3}\gg \Lambda_{\rm QCD}^2$ dependence of an emergent saturation scale controlling the nonlinear dynamics of saturation. Likewise, there there is a powerful interplay between contributions to the proton spin at small $x$ and the physics of gluon saturation. 

Ensuring that the EIC can realize its enormous promise and deliver on the discovery of gluon saturation requires 
both broad and focused collaborative theoretical research including identification and computation of observables sensitive to gluon saturation in DIS off 
polarized protons ($e+p$) and heavy nuclei ($e+A$), along with observables from hadron collider experiments. This effort also requires robust end-to-end calculations that minimize known uncertainties on each of these observables with an ambitious goal of $<10\%$ accuracy, sufficient for the unambiguous characterization of the gluon-dominated small $x$ regime in protons and nuclei. Not least, new and potentially transformative ideas (and their empirical consequences) connecting the physics of gluon saturation to the 
intrinsically non-perturbative physics of color confinement and chiral symmetry breaking in QCD need to be explored. 

The ambitious goal of precision in data-theory comparisons at small $x$ is driven by the significant progress achieved in recent years in 
next-to-leading order (NLO) computations of process-dependent ``impact factors" for key final states and 
advances in computing the  small-$x$ renormalization group leading logarithm BK~\cite{Balitsky:1995ub,Kovchegov:1999yj} and JIMWLK equations~\cite{Jalilian-Marian:1997ubg,Iancu:2000hn} to next-to-leading logarithmic (NLL) accuracy. Combining the developments in impact factors and small $x$ evolution for a number of final states enables us to reach the desired $O(\alpha_S^2)$ cross section accuracy, corresponding to the required $10\%$ figure of merit.

In DIS, formal expressions for NLO impact factors have been derived for key observables such as inclusive structure functions \cite{Balitsky:2010ze,Beuf:2017bpd}; heavy quark structure functions \cite{Beuf:2021srj};  diffractive dihadron, dijet and exclusive vector meson production \cite{Boussarie:2016ogo,Boussarie:2016bkq,Mantysaari:2022kdm,Fucilla:2022wcg}; single inclusive hadrons \cite{Bergabo:2022zhe}; and inclusive dijet, dihadron \cite{Caucal:2021ent,Caucal:2022ulg,Bergabo:2022tcu,Bergabo:2023wed}, and hard photon \cite{Roy:2019hwr} final states.  Recently proposed observables such as coherent inelastic dijet production, photon-jet and lepton-jet correlations, as well as nucleon energy correlators, remain to be studied to NLO accuracy~\cite{Iancu:2021rup,Kolbe:2020tlq,Tong:2022zwp,Liu:2023aqb}. However in many cases, even where formal expressions exist, the impact factors have not been explicitly evaluated, primarily due to their numerical complexity. Combining analytical progress with numerical implementation will be an important collaborative task. 

A key aspect of such implementation is to combine advances in computing process-dependent impact factors with universal small $x$ evolution in a consistent manner. There are still a number of conceptual questions involved in this matching that have generated new theoretical work. The issues involved pertain to the poor treatment of the collinear regime; resummation of higher-order terms was required to cure the problem. 
Similar to linear BFKL~\cite{Fadin:1975cb,Kuraev:1976ge,Kuraev:1977fs,Balitsky:1978ic}, the renormalization group (RG) improved treatment of collinear logs, discussed in the context of the CGC EFT in Ref.~\cite{Lappi:2016fmu,Ducloue:2019ezk}, is essential for robust predictions. 
Unless these large logarithmic contributions are properly accounted for, the NLO-level results can lead to unphysical (negative) cross sections \cite{Stasto:2014sea}. It is only recently that the first computations taking all these elements into account in the context of back-to-back inclusive dijets have become available~\cite{Caucal:2022ulg}.

Such systematic computations indicate the importance of parton lifetime constraints on RC evolution at small $x$, known to regulate the behavior of the NLL BFKL~\cite{Fadin:1998py,Ciafaloni:1998gs} equation. A full understanding of its impact on the NLL JIMWLK RG equations~\cite{Balitsky:2013fea,Kovner:2014lca} remains to be understood although there is promising work in this direction~\cite{Ducloue:2019ezk}.  There is a powerful spacelike-timelike correspondence~\cite{Mueller:2018llt} first discussed in the context of the relation of non-global logarithms in $e^+e^-$ collisions 
to small $x$ evolution~\cite{Hatta:2013iba}, and later exploited to compute key pieces of the NNLO RG evolution equations~\cite{Caron-Huot:2016tzz}. This connection has led to a powerful synergy between the small $x$ and ``amplitudes" communities in developing precision tools which have the potential to significantly enhance the EIC theory alliance (EICTA)~\cite{Travaglini:2022uwo}.

Sub-eikonal corrections to the  eikonal approximation employed in CGC calculations will extend its applicability to higher $p_T$ and improve its accuracy at small $x$~\cite{Jalilian-Marian:2017ttv,Jalilian-Marian:2018iui,Jalilian-Marian:2019kaf,Boussarie:2021wkn,Boussarie:2020fpb}. 
Such sub-eikonal corrections can be calculated systematically either at the level of propagators~\cite{Altinoluk:2020oyd,Altinoluk:2021lvu} or of observables like the DIS dijet cross section~\cite{Altinoluk:2022jkk}.  The study of the back-to-back dijet limit will clarify the matching between the TMD formalism, supplemented by higher-twist power corrections, and the CGC formalism, supplemented by sub-eikonal power corrections.   

DGLAP-based fits of helicity PDFs are plagued by extrapolation issues into the small-$x$ regime~\cite{DeFlorian:2019xxt,Borsa:2020lsz}.   
Small-$x$ helicity evolution equations, the Kovchegov-Pitonyak-Sievert--Cougoulic-Tarasov-Tawabutr (KPS-CTT) equations, involving the {\em polarized dipole amplitude}, 
were derived in~\cite{Kovchegov:2015pbl,Kovchegov:2016zex,Kovchegov:2017lsr,Kovchegov:2018znm,Cougoulic:2022gbk}.  The first implementation of the older KPS equations extracted the $g_1$ structure function from the world's polarized DIS data~\cite{Adamiak:2021ppq}. 
The growth of helicity PDF studies will be aided tremendously by the EIC-TA. For example, compared to previous work fitting DIS double-spin asymmetries~\cite{Adamiak:2021ppq} with the (unpolarized) denominator determined from  DGLAP fits, improved self-consistent fits should employ the small $x$ unpolarized RG equations discussed above. 
 Processes such as polarized SIDIS and polarized proton-proton collisions, need to be incorporated into the framework. To distinguish individual flavor contributions,  double-log approximation large-$N_c$ solutions~\cite{Adamiak:2021ppq} currently employed should be replaced by results in the large-$N_c$\&$N_f$ limit~\cite{Kovchegov:2020hgb}.  
Similarly, improved determination of helicity-dependent initial conditions should replace the {\it ad hoc} fitting procedure in Ref.~\cite{Adamiak:2021ppq}.  Saturation corrections to the KPS-CTT equations~\cite{Kovchegov:2021lvz} from the unpolarized dipole correlator are required to study their effect on parton spin. Predictions for the proton orbital angular momentum  carried by small-$x$ quarks and gluons are feasible~\cite{Kovchegov:2019rrz}.  The polarized dipole amplitude approach lends itself to systematic improvements within a global analysis framework. 
An important issue which is not addressed by the above analyses is the role of the chiral anomaly. Work in this direction suggests that the quark helicity is proportional to the QCD topological susceptibility~\cite{Narison:1998aq,Tarasov:2020cwl,Tarasov:2021yll}. A similar effect due to the trace anomaly has been uncovered in deeply virtual Compton scattering (DVCS)~\cite{Bhattacharya:2022xxw}. These anomaly studies connect the small $x$ community to researchers working on various aspects of non-perturbative QCD that include lattice QCD and chiral perturbation theory.

Single forward emission in inclusive as well
as exclusive channels gives us  direct access to the unintegrated gluon distribution (UGD) in the proton and BFKL evolution at small-$x$. This BFKL-based approach to UGDs was previously applied to: forward emission of light vector mesons at HERA~\cite{Anikin:2009bf,Anikin:2011sa,Besse:2013muy,Bolognino:2018rhb,Bolognino:2019pba,Bolognino:2021niq,Cisek:2022yjj,Luszczak:2022fkf,Celiberto:2019slj,Bolognino:2018mlw,Bolognino:2019bko,Bolognino:2021gjm,Bolognino:2022uty,Bolognino:2022ndh}; heavy quarkonia~\cite{Bautista:2016xnp,ArroyoGarcia:2019cfl,Hentschinski:2020yfm}; and forward Drell--Yan detections at LHCb~\cite{Motyka:2014lya,Motyka:2016lta,Brzeminski:2016lwh,Celiberto:2018muu}. The EIC can potentially unveil connections between UGDs and the unpolarized and Boer--Mulders gluon TMDs~\cite{Hentschinski:2021lsh,Nefedov:2021vvy,Celiberto:2021zww,Bolognino:2021niq}. Likewise, excellent agreement is obtained between the CGC EFT and HERA data on proton $F_2$ and $F_L$ \cite{Beuf:2020dxl} and heavy quark structure functions~\cite{Hanninen:2022gje} as well as for forward single inclusive hadron production data at RHIC and the LHC \cite{Shi:2021hwx}. 


The  onset of gluon saturation should exhibit distinctly different systematics from those seen in the absence of saturation. Such differences could be striking in exclusive vector meson production off large nuclei \cite{Mantysaari:2017slo}.
In particular, one expects the scaling behavior of vector meson production cross sections in both nuclear mass number, $A$, and photon virtuality, $Q^{2}$, to be strongly modified due to 
saturation effects. Recent simulations with the Sar{\em t}re \cite{Toll:2013gda,Toll:2012mb} Monte Carlo event generator confirm this scaling in a realistic EIC kinematic setup, where the results are obtained via cross section pseudo-data collected by Sar{\em t}re \cite{Matousek:2022enl}, and then parsed through 
smearing functions that emulate proposed EIC detector resolution; theoretical and experimental challenges are detailed in 
Ref.~\cite{Matousek:2022enl,AbdulKhalek:2021gbh}. 
 
An interesting signature of  saturation is geometrical scaling (GS) in exclusive vector meson production,  inspired by previous work on inclusive DIS \cite{Stasto:2000er} 
observed at HERA \cite{Golec-Biernat:1998zce,Golec-Biernat:1999qor,Marquet:2006jb},as well as in proton and pion structure at small $x$ at HERA \cite{Kumar:2022kww}, hadronic collisions at the LHC \cite{McLerran:2010ex,McLerran:2010wm}, and perhaps also in heavy-ion collisions at RHIC and the LHC \cite{Khachatryan:2019uqn,Khachatryan:2022qrc}. 
Based on these examples, GS is expected to exist in exclusive vector meson production in $e+A$ (and possibly in $e+p$) at the EIC \cite{Ben:2017xny,Kowalski:2006hc}.  Sar{\em t}re can be used to generate events and perform cross section calculations as a function of the transverse momentum of the produced vector mesons.

Recent phenomenological studies dedicated to photoproduction of $J/\psi$ and $\psi(2s)$ in ultraperipheral collisions at the LHC indicate that the ratio of their cross sections can distinguish linear from non-linear small $x$ evolution \cite{Hentschinski:2020yfm}. At the EIC, a similar result is expected from varying $A$. To explore the full consequences of non-linear small $x$ evolution, it will be  beneficial to complement EIC measurements by LHC forward physics results which, albeit limited in precision relative to the EIC, have a wider $x$ range. See Ref.~\cite{Hentschinski:2022xnd} for a recent summary of possible measurements. 

The Good-Walker paradigm relates coherent photo/electroproduction to the average nuclear configuration where $d\sigma/dt$ is sensitive to the transverse distribution of gluons in the nuclear target \cite{Klein:2019qfb}.  Incoherent photoproduction is, in turn, sensitive to event-by-event fluctuations in the target, including gluon hotspots \cite{Miettinen:1978jb}.  Unfortunately, the Good-Walker paradigm is, by nature, a lowest order formalism which fails in some cases \cite {Klein:2023zlf}.  
For large (negative) values of $t$, the incoherent cross section is nevertheless proportional to the fluctuations in the initial state of the target wave function. In the dense saturated kinematic regime, these fluctuations are expected to be suppressed \cite{Cepila:2016uku, Mantysaari:2018zdd, Kumar:2022aly}. The EIC 
can therefore trace the onset of saturation in the suppression of the incoherent cross section in exclusive diffraction at intermediate and large values of $|t|$.

Exclusive production of vector mesons, photons (including DVCS) or other final states allows for unique measurements but introduces additional theoretical problems in understanding the Pomeron.  To lowest order, the Pomeron is a color singlet combination of two gluons.  However recent theoretical calculations of exclusive $J/\psi$ photoproduction  found several surprises: a large contribution from quarks (partly due to a significant cancellation in the gluon components) and a strong scale dependence \cite{Eskola:2022vpi}. Additional calculations are needed to understand the implications of this result and to determine how to best use this data in determining nuclear PDFs. 

Quantum coherence \cite{Kopeliovich:2001xj} and color transparency (CT) \cite{Kopeliovich:1993gk} is conveniently studied in diffractive photo- and electro-production of heavy quarkonia \cite{Kopeliovich:2022jwe} 
 within a Greens function formalism \cite{Kopeliovich:2001xj,Kopeliovich:2022jwe}; this formalism has also been applied to exclusive production of light vector mesons \cite{Kopeliovich:2001xj}, diffractive DIS and DVCS \cite{Kopeliovich:2010sa}. Since both quantum coherence and color transparency are features of the CGC formalism, it will be interesting to further explore the connections between apparently different formalisms and arrive a common understanding. A recent review of the phenomenological status of gluon saturation measurements at colliders can be found in \cite{Morreale:2021pnn}.

The two most widely used initial conditions for small $x$ evolution are those of the Golec-Biernat--W\"usthoff (GBW) \cite{Golec-Biernat:1998zce,Golec-Biernat:1999qor} and the McLerran--Venugopalan (MV) models \cite{McLerran:1993ka,McLerran:1993ni}. The former captures key features of saturation but does not match smoothly to LO perturbative QCD. 
The latter is more robust but is valid strictly for large nuclei. 

How to go beyond the GBW and MV models to extract reliable initial conditions for multipole correlators at $x\sim 10^{-2}$ is an outstanding question.  Fluctuation-driven non-Gaussian effects derived from analogy of ``BK dipole evolution" to wavefront propagation in statistical mechanics provide useful guidance in going beyond the MV model \cite{Mueller:2014fba,Caucal:2021lgf} and can be tested in diffractive final states at the EIC \cite{Le:2020zpy}.

A promising first principles approach for light nuclei is to compute color charge correlators on the light front \cite{Dumitru:2018vpr,Dumitru:2020gla,Dumitru:2021tqp} which can be constrained by DIS data at large $x$ \cite{Dumitru:2019qec,Dumitru:2021tvw}.  Another such promising approach is to employ the techniques of Large Momentum EFT (LaMET) \cite{Ji:2020ect,Zhang:2018diq} to compute the energy dependence of $p_T$-dependent parton distributions from Lattice QCD \cite{Shanahan:2021tst} or extract color charge correlators.  Reaching down to $x\sim 10^{-2}$ is however challenging since it requires high resolution on the lattice or new ideas to circumvent the need for very small lattice spacing.

Small $x$ physics and gluon saturation have interesting conceptual and practical connections to several subfields of physics. In the high energy Regge limit at large $N_c$, the LL BFKL equation has a rich mathematical structure and can be understood as dual to the XXX spin chain with negative spin which is an integrable model that 
is solvable by the Bethe Ansatz. This mapping of small $x$ dynamics is valuable for providing insight into the role of entanglement in DIS~\cite{Zhang:2021hra}. The role of quantum entanglement and quantum information science (QIS) in DIS at small $x$ has been discussed recently in Refs.~\cite{Kharzeev:2017qzs,Duan:2021clk,Dumitru:2022tud,Hentschinski:2022rsa}.  It was recently suggested that gluon saturation can be understood  as a maximally-occupied state whose microstates saturate the universal Bekenstein bound~\cite{Dvali:2021ooc}. QIS studies are a new direction of EIC physics appropriate for the EIC-TA and exhibit the potential for productive synergy with other areas of physics.

The small $x$ studies undertaken by the EIC-TA are also valuable for QCD studies at the LHC, particularly for understanding the role of multi-parton interactions (MPIs) in hard processes. Small $x$ has played a key role in understanding the initial state and the thermalization process in heavy-ion collisions~\cite{Berges:2020fwq}. Prior to the EIC, there has been a significant amount of data taken at RHIC and the LHC that are sensitive to small $x$ physics and gluon saturation. The EIC-TA will interact with the heavy-ion community in analyzing these data and incorporating them in global analyses. This is a primary goal of the recently approved SURGE (Saturated Glue) DOE topical collaboration which will have considerable overlap with the goals of the EIC-TA. 

Small $x$ QCD also places important constraints on the astrophysics of cosmic neutrinos~\cite{Anchordoqui:2006ta,Cooper-Sarkar:2011jtt,Garcia:2020jwr,Candido:2023utz}. Conversely, measurements at cosmic neutrino observatories such as ICECUBE can help distinguish between differing frameworks of QCD evolution at small $x$~\cite{Bhattacharya:2016jce}.








